AUDITPLAN: Commit, Then Answer for Auditable Safety Alignment

Safety tuning pipelines judge only the final answer, which makes it difficult to distinguish robust refusal from two undesirable shortcuts: blanket refusal on benign requests and polished but unfaithful safety rationales that do not actually constrain the answer. We propose AUDITPLAN, a single-model plan-then-answer approach where the model first emits a compact structured safety plan and then answers conditioned on it. The plan records a threat label, intended action, and explicit constraints, enabling machine-checkable auditing while remaining hidden from users at deployment. We train this behavior with supervised fine-tuning followed by reinforcement learning with FAITHGATE, a reward-gating objective that grants answer reward only when the safety plan is correct. This discourages safe-looking but unfaithful behavior and promotes tighter plan-answer coupling. Across Qwen backbones, AUDITPLAN improves both robustness and auditability: on Qwen2.5-3B-Instruct, FAITHGATE reduces ASR from 24.0% to 11.6%, LSR from 1.0% to 0.36%, and over-refusal from 11.0% to 2.0%, outperforming answer-only RL, free-form explanation, and weighted-sum structured rewards. Similar trends hold for Qwen2.5-1.5B-Instruct. Larger-model confirmation runs on Qwen-3-4B-Instruct and Qwen2.5-7B-Instruct preserve the same trend suggesting that explicit internal commitments can make safety alignment more faithful, robust, and auditable.

==> fig_relative_tikz.tex <==
\definecolor{APBlueBar}{RGB}{66,122,171}
\definecolor{APOrangeBar}{RGB}{238,134,38}
\begin{tikzpicture}[x=0.064cm,y=0.56cm]
\node[font=\bfseries\small, align=center] at (50,6.4) {\gate\ relative improvement over weighted-sum 3B baseline};
\draw[->, black!65] (0,0.45) -- (100,0.45);
\foreach \x in {0,20,40,60,80,100}{\draw[black!20] (\x,0.55) -- (\x,5.85); \node[below, font=\tiny] at (\x,0.35) {\x};}
\foreach \name/\val/\yy/\col in {ASR/51.9/5.2/APBlueBar, LSR/64.0/4.4/APBlueBar, ORR/82.1/3.6/APBlueBar, PAA/24.5/2.5/APOrangeBar, PAC/22.9/1.7/APOrangeBar, PS/30.8/0.9/APOrangeBar}{
  \node[anchor=east, font=\scriptsize] at (-1,\yy) {\name};
  \fill[\col] (0,\yy-0.23) rectangle (\val,\yy+0.23);
  \node[anchor=west, font=\scriptsize] at (\val+2,\yy) {\val\%};
}
\node[anchor=west, font=\tiny, text=APBlueBar] at (4,6.0) {security/helpfulness: lower ASR, LSR, ORR};
\node[anchor=west, font=\tiny, text=APOrangeBar] at (55,6.0) {auditability/faithfulness: higher PAA, PAC, PS};
\end{tikzpicture}

